Real or Not Real, that is the Question

While generative adversarial networks (GAN) have been widely adopted in various topics, in this paper we generalize the standard GAN to a new perspective by treating realness as a random variable that can be estimated from multiple angles. In this generalized framework, referred to as RealnessGAN, the discriminator outputs a distribution as the measure of realness. While RealnessGAN shares similar theoretical guarantees with the standard GAN, it provides more insights on adversarial learning. Compared to multiple baselines, RealnessGAN provides stronger guidance for the generator, achieving improvements on both synthetic and real-world datasets. Moreover, it enables the basic DCGAN architecture to generate realistic images at 1024*1024 resolution when trained from scratch.

==> secs/ablation.tex <==
\vspace{-3mm}
\subsection{Ablation Study}
The implementation of \emph{RealnessGAN} offers several choices that also worth digging into. On synthetic dataset, we explored the relationship between the number of outcomes and $G$'s update frequency. On real-world dataset, apart from evaluating \emph{RealnessGAN} as a whole, we also studied the affect of feature resampling, different settings of $\cA_0$ and $\cA_1$ and choices of $G$'s objective. 

\begin{minipage}{\textwidth}
\vspace{-3mm}
\begin{minipage}[b]{0.45\textwidth}
\centering
\small
\captionof{table}{Minimum (min), maximum (max), mean and standard deviation (SD) of FID on CelebA using different anchor distributions, calculated at 20k, 30k, ... iterations.}
\label{tab:anchor_shape}
\begin{tabular}{ccccc}
\toprule
$\KL( \cA_1 \Vert \cA_0)$           & Min                       & Max                       & Mean                      & SD                       \\ \midrule
1.66       & 31.01 & 96.11 & 40.75 & 11.83 \\
5.11 & 26.22                     & 87.98                     & 36.11                     & 9.83                      \\
7.81       & 25.98                     & 85.51                     & 36.30                     & 10.04                     \\ 
11.05    & 23.51                     & 81.30                     & 30.82                     & 7.61      \\ \bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[b]{0.45\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/update/ablation_resampling_update.pdf}
\captionof{figure}{Training FID curves of \emph{RealnessGAN} with and without feature re-sampling.}
\label{fig:ablation_resample}
\vspace{-10mm}
\end{minipage}
\end{minipage}

\begin{figure}[t]
\centering
\includegraphics[width=0.6\textwidth]{figs/update/G_objective_snapshot.pdf}
\caption{Samples generated by \emph{RealnessGAN} trained with the ideal objective (\eqref{eq:g_objective1}).
Top-row: samples when $\KL( \cA_1 \Vert \cA_0) = 11.05$. Bottom-row: samples when $\KL( \cA_1 \Vert \cA_0) = 33.88$.}
\label{fig:ablation_GLOSS2}
\end{figure}


\begin{minipage}{\textwidth}
\vspace{-1mm}
\begin{minipage}[b]{0.5\textwidth}
\centering
\small
\captionof{table}{FID scores of $G$ on CIFAR10, trained with different objectives.}
\label{tab:g_objectives}
\begin{tabular}{cc}
\toprule
G Objective  &  FID  \\ \midrule
Objective1 (\eqref{eq:g_objective1}) & 36.73 \\
Objective2 (\eqref{eq:g_objective2}) & 34.59 \\
Objective3 (\eqref{eq:g_objective3}) & 36.21 \\
DCGAN & 38.56 \\ 
WGAN-GP & 41.86 \\
LSGAN & 42.01 \\
HingeGAN & 42.40 \\ \bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[b]{0.45\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/update/ablation_G_objective_update.pdf}
\captionof{figure}{Training curves of \emph{RealnessGAN} on CelebA using objective2 (\eqref{eq:g_objective2}) and objective3 (\eqref{eq:g_objective3}).}
\label{fig:curve_g_objectives}
\vspace{-15mm}
\end{minipage}
\end{minipage}



\noindent \textbf{Feature Resampling.}
Fig.\ref{fig:ablation_resample} shows the training curves of \emph{RealnessGAN} with and without feature resampling. It can be noticed that despite the results are similar, feature resampling stabilizes the training process especially in the latter stage. 

\noindent \textbf{Effectiveness of Anchors.}
Tab.\ref{tab:anchor_shape} reports the results of varying the KL divergence between anchor distributions $\cA_0$ and $\cA_1$. The FID score indicates that, as the KL divergence between $\cA_0$ and $\cA_1$ increases, \emph{RealnessGAN} tends to perform better, which verifies our discussion in Sec.\ref{sec:method_discussion} that a larger difference between anchor distributions imposes stronger constraints on $G$. To further testify, two different pairs of anchors with similar KL divergences ($11.95$ and $11.67$) are exploited and they yield comparable FID scores ($23.98$ and $24.22$). 

\noindent \textbf{Objective of G.}
As mentioned in Sec.\ref{sec:method_discussion}, theoretically, the objective of $G$ is $\max_G \Ebb_{\vx \sim p_g}[\KL( \cA_0 \Vert D(\vx))]$. 
However, in practice, since $D$ is not always optimal, we need either a pair of $\cA_0$ and $\cA_1$ that are drastically different, or an additional constraint to aid this objective. 
%As mentioned in Sec.\ref{sec:implementation}, two alternative choices for the additional constraint are provided, resulting in \eqref{eq:g_objective2} and \eqref{eq:g_objective3}.
Fig.\ref{fig:ablation_GLOSS2} shows that, with the ideal objective alone, when the KL divergence between $\cA_0$ and $\cA_1$ is sufficiently large, 
on CelebA we could obtain a generator with limited generative power.
On the other hand, by applying constraints as discussed in Sec.\ref{sec:implementation}, 
$G$ can learn to produce more realistic samples as demonstrated in Fig.\ref{fig:real_snapshots}. 
Similar results are observed on CIFAR10,
where \emph{RealnessGAN} obtains comparable FID scores with and without constraints, 
as shown in Tab.\ref{tab:g_objectives}.
Fig.\ref{fig:curve_g_objectives} also provides the training curves of \emph{RealnessGAN} on CelebA using these two alternative objectives. 
%Tab.\ref{tab:g_objectives} includes FID scores of $G$ on CIFAR10, FID scores obtained by training with
% the ideal and alternative objectives are: 36.73 (\eqref{eq:g_objective1}), 34.59 (\eqref{eq:g_objective2}) and 36.21 (\eqref{eq:g_objective3}). 
%Results on CIFAR10 
%indicates that, with or without adding constraints, the objective of \emph{RealnessGAN} performances of different objectives are comparable on simpler tasks.

% \begin{minipage}{\textwidth}
% \vspace{-5mm}
% \begin{minipage}[b]{0.45\textwidth}
% \centering
% \small
% \vspace{-5mm}
% \captionof{table}{\small FID score of RealnessGAN trained with different objectives of $G$ on CIFAR10. With or without adding the constraint, performances of different objectives are comparable on simple tasks.}
% \label{tab:g_objectives}
% \begin{tabular}{lc}
% \hline
% Objective & FID \\ \hline
%  Ideal Objective (\eqref{eq:g_objective1}) & $36.73$ \\
%  Objective 2 (\eqref{eq:g_objective2}) & $34.59$ \\
% Objective 3 (\eqref{eq:g_objective3}) & $36.21$ \\
% \hline
% \end{tabular}
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.45\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figs/update/ablation_G_objective_update.pdf}
% \captionof{figure}{\small Training curves of RealnessGAN on CelebA using objective2 (\eqref{eq:g_objective2}) and objective3 (\eqref{eq:g_objective3}).}
% \label{fig:curve_g_objectives}
% \vspace{-12mm}
% \end{minipage}
% \end{minipage}




